Controllable Citation Sentence Generation with Language Models

Citation generation aims to generate a citation sentence that refers to a chosen paper in the context of a manuscript. However, a rigid citation generation process is at odds with an author's desire to control specific attributes, such as 1) the citation intent, e.g., either introducing background information or comparing results, and 2) keywords that should appear in the citation text. To provide these degrees of controllability during citation generation, we propose to integrate the manuscript context, the context of the referenced paper, and the desired control attributes into a structured template and use it to fine-tune a language model (LM) via next-token prediction. We then utilize Proximal Policy Optimization to directly optimize the LM in favor of a high score of our proposed controllability metric. The proposed workflow harmoniously combines citation attribute suggestion and conditional citation generation into one LM, allowing for better user control.

==> bkup.tex <==
% aims to generate a citation sentence that cites and discusses the target paper in the context of the manuscript.
% 2. Background: How was citation generation addressed previously?
% It 

% The task of citation text generation is considered as a summarization problem: the summarizer takes as input information about the manuscript being written and the cited paper, and automatically generates a citation sentence that discusses the cited paper in the context of the manuscript.

% The citation text generation task is usually treated as an abstract summarization problem: a sequence-to-sequence model takes as input the contextual sentences from the manuscript and the abstract of the cited paper, and outputs a citation sentence.
% This setup oversimplifies the actual situation of citing a paper, ignoring the fact that the way a paper is cited can vary depending on various conditions, such as 1) the citation intent, e.g., introducing background or comparing results; 2) keywords that prompt the citation of a specific paper; and 3) relevant sentences in the full text of the cited paper, which may contain details that the author wants to cite. The citation generation model trained under such a simplified setting cannot adjust the generated citations according to the conditions specified by the user.
% In this work, we propose a conditional citation generation system that uses conditions as an additional source of input when training a Bart-based abstractive summarizer. We further develop a pipeline to infer the citation intent and propose tentative keywords and relevant sentences, which the user can select to tune the generation.
% Our framework gives users a higher degree of control in generating citations and achieves better user satisfaction in our human evaluations compared to citation generation models without condition awareness.




% The purpose of citation generation is to generate a citation sentence to cite and discuss a paper in the citing context. In recent work, this task has been treated as an end-to-end sequence-to-sequence problem, 

% this task is usually considered as a sequence-to-sequence problem, where the output is the citing sentence, the input contains several sentences before and after the citation sentence as the local context, and the abstract of the cited paper as the global context. Such an input setting deviates from the real scenario of scientific writing due to the lack of two additional sources of knowledge: 1) the citation point, such as certain keywords that motivate the citing of a certain particular paper.
% % which is the main focus that motivates the citation of a particular paper. Authors may already have some keywords before writing citation sentences, as these keywords usually explain why the corresponding paper is cited, such as explaining a term or supporting a concept, where the term or concept is the citation point; 
% and 2) top relevant sentences in the full text of the cited paper, which may exclusively contain detailed information that the authors want to cite.
% % and which may not be included in the abstract.
% In this work, we show that the performance of citation generation is significantly improved after explicitly introducing this additional knowledge into the language model trained on the citation generation task.
% % , the quality of the generated citation text is significantly improved, with improved accuracy and consistency with respect to ground truth citation sentences.
% Furthermore, to cope with the situation where no additional knowledge is explicitly provided, we propose a framework that extracts the citation point from the local and global context and relevant sentences from the full text of the target paper and augments citation generation with them as additional knowledge. Our framework outperforms the citation generation model without knowledge augmentation in both ROUGE and human evaluation.


% The purpose of the citation generation task is to generate a citation sentence that cites and discusses the target paper in the context of the manuscript, which serves as an assitive tool for authors to cite papers in scientific writing.
% In scientific writing, a common case is when authors need to cite a paper to support a certain point, to provide background information and to compare the results [CIT REF paper]. 

 The first two components can be considered as the local context, and the abstract of the cited paper can be treated as the global context.
 
 A sequence-to-sequence model based on RNN-based pointer generator is constructed, where the attention for copy mechanism consists of the cross attention between the local context and the global context.
 
 
where a summarization system automatically generates a sentence to cite and discuss a paper in the citing context, given the information of the manuscript being written and the cited paper.
a sequence-to-sequence model takes as input the contextual sentences from the manuscript and the abstract of the cited paper and outputs a citation sentence.

% This setup oversimplifies the actual situation of citing a paper, ignoring the fact that the way a paper is cited can vary depending on various conditions, such as 

% The citation generation model trained under such a simplified setting cannot adjust the generated citations according to the conditions specified by the user.


% cite a paper 

% This paper proposes an approach to automatically generating a related work section by comparing the main text of the paper being written with the citations of other papers that cite the same references

% In \cite{chen_automatic_2019} the model was trained to generated related works section. The generated text of the paper is a general summarization of the work which usually serves as the background information.  

where the input text consists of two components: 1) three sentences before and after the ground-truth citation sentence that we aim to generate, which can be treated as the local context and the abstract of the cite paper as the global context. 


% These keywords may lead to different citing sentences even if the cited paper is the same and the local context is similar. 
% [Find an example HERE from the dataset]


% This motivates our work of designing a more 

In this case, authors may want to alter the  

% Different intents and topical keywords lead to different citing sentences even if the cited paper is the same and the context is similar (Figure \ref{fig:example-multi-intent-in-one-para}), which is hard for 

% However, in previous works the information on the citation intent, topical keywords and relevant sentences are usually not explicitly given, and it is hard for the model in infer these information solely based on the context in the manuscript and the cited paper's information. For example, different topical keywords and intents lead to different citing sentences even if the cited paper is the same and the context is similar (Figure \ref{fig:example-multi-intent-in-one-para}).


% authors can cite the same paper multiple times in one paragraph with varied intentions and topical keywords

% These keywords may lead to different citing sentences even if the cited paper is the same and the local context is similar.

% often have a clear intention before citing a paper, such as comparing results or presenting background information. Second, authors can have some topical keywords in mind before writing citation sentences, and these keywords usually guide the citation of the corresponding paper, such as explaining a term or supporting a concept. In addition, authors may first pinpoint the most relevant sentences in the cited papers' full text, and then start to write a sentence based on that, especially when authors want to cite a paper to compare the certain experiment results in the target paper

% Third, the abstract may contain insufficient information to produce the citation sentence. Especially when authors want to cite a paper to compare the certain experiment results in the target paper, which may be only briefly mentioned in the abstract but more detailed described in the full text. 
% Instead, before authors write citation sentences, they may first pinpoint the most relevant sentences in the cited papers' full text, and then start to write a sentence based on that.
% Missing the full text can lead to generation of ambiguous and less accurate citation text. 

% user typically have a clear intention, topical keywords and target sentence thta want to discuss before they write a sentence. While the former part cannot be fully automated or at leadt allow users to intervene the generation on their will.  A less controllable cit gen model will limit it usage in scinetific writing where authors can take many ietrative round of fintuning until the generated citation sentence is ready to be put into the manuscript

% Such as "co-occurrence of words" v.s "co-occurence of sentences". 
% []Find some example that  the key information is not included in the abstract]
% In this work, we want to explore the following questions:
% \begin{itemize}
%     \item  Will the performance of citation generation improved if 
% we know the additional knowledge of  citing points (keywords) and relevant sentences from the full text?
%     \item How to improve the citation generation performance we have only local, global context and cited paper's full text, but without explicitly provided keywords and relevant sentences>
% \end{itemize}

% In previous works the information on the citation intent, topical keywords and relevant are either not explicitly given or not covered. Generation of citation sentence is a one-shot manner, where users can hardly fine-tune the generation on thir will, which we believe limits the usefulness of citation generation models in real-life writing.


% What we do?
% We proposal a citation generation framework which is tunable based on user input. Instead of fully-automize the generation process, we leave space for users to empower the final generation the yield more satisfactory results.


% To answer these questions, we adapt the attention-based language model T5 which is pretrained on XXX tasks, and proved to be able to take multiple sources of texts as input and perform well in a multi-task training scheme. 
% We first train a basic version of T5 which takes local context, cited paper's abstract as input, as a baseline;

% To test the influence of keywords, we extract from the local and global context up-to two key phrases which has a maximum ROUGE similarity to the citation sentence, to imitate the situation where the authors know a few keywords before writing citation sentence. We  add these keywords as an additional source of input to the language model, and compare the performance with the baseline model;

% To test the influence of knowing the relevant sentences, we use the citing sentence as query, to get top k most similar (in terms of cosine similarity) sentences to use them as additional input, and compare with baseline model.

% Our experiments results show that knowing keywords/relevant sentences boost the performance / generation accuracy,  the quality of the generated citation text is significantly improved, with improved accuracy and consistency with respect to ground truth citation sentences.


% Motivated by this results, we propose a pipeline to proactively extract keywords from local / global context, and extract relevant sentences from the full-text, and use them as augmented knowledge to enhance the citation generation model. The experiments results indicates an effective utilization of the addition knowledge.

% Potential XXX: use the keywords / relevant sentences as a way for post processing, to select sentences from beam search results or top-p sampling.

% Contribution of this work:
% \begin{itemize}
%     \item Evaluate the influence of additional knowledge of keywords and relevant sentences;
%     \item propose a pipeline capable of automatically extract tentative keywords and relevant sentences that can be used to augument the input, [] as well as fine-grain the decoding process ].
%     \item we propose a new dataset, which eliminate the potential entanglement between training and test set, reducing the probability of overfitting especially for citation generation model based on large language models.
% \end{itemize}

% with original input to enforce the generation process conditioned on the atrributes to achieve the manupulation of generation, while in our work we apply this idea to a abstractive summarization task with flexibly defined attributes, e.g. we only have three labels for intent, following the classification work \cite{cohan-etal-2019-structural}; we treat keywords and relevant sentence as attributes without pre-clsutering them.
% % e.g. except ciation intent, which we calssfied into three types, we do not classfy

% \subsubsection{Keyword Suggestion and Relavant sentences suggestion}
% similar to KeyBERT \cite{}, although it is unserpervised
% SciBERT model --> condition text embedding -> keyword/sentence embeddings , ranking them based on cosine similarity!

% intuition: put keywords more related to citation generation ranked higher in order

% how to train LOSS. Triplet loss:
% Sort keywords according to the rouge 1,2 F scores w.r.t the ground truth citation sentence, get the order (ranking), Thoese with the same rouge scores obtain the same rank, then we constrcut the triplet loss following MatchSUM \cite{}
% Loss function here!

% Sentence selection are simialar except we are comparing the simalrity between contexual text embedding and full text sentence embeddings


% contextual text or keywords into an embedding. The encoding is achieved by averaging the last hidden state of all tokens in a text $S$ to produce the embedding $e_S$.


% mean of ROUGE-1\&2 F1 scores between the keyword and the target citation sentence. Keywords that 

% Following \citet{zhong_extractive_2020}, we use a siamese SciBERT to encode the contextual text or a keyword into an embedding by averaging the last hidden states of all tokens in the text. We fine-tune the SciBERT model so that the embeddings of keywords more relevant to the target citation sentence have higher cosine similarities to the embedding of the contextual text, so that we can use the contextual text as a query to rank the keywords based on the cosine similarity.

% We use triplet loss to fine-tune the SciBERT model. Given a list of candidate keywords.


% \begin{table}
% \centering
% \resizebox{\linewidth}{!}{ 
% \begin{tabular}{lcccc}
% \toprule
% Model &  R-1 & R-2 & R-L & BERTScore \\
% \midrule
% % \multicolumn{4}{l}{ \small{\textbf{citation attributes as oracle extractive summary, no contextual text}}} \\[0.2em]
% % relevant keywords & 28.52 & 8.75 & 20.40 & \\
% % relevant sentences & 37.15 & 13.94 & 25.09 & \\
% % \midrule
% \multicolumn{5}{l}{ \small{\textbf{contextual text as input for generation, no citation attributes}}} \\[0.2em]
% PTGEN-Cross$^\dagger$ & 24.96  &  4.14 & 18.51 & .8547\\
% BART-large & 29.63 & 7.56 & 22.53 & .8758\\
% \midrule
% \multicolumn{5}{l}{ \small{\textbf{both contextual text and citation attributes as input for generation}}} \\[0.2em]
% BART-large-CCG \\
%   w/ intent $i$  & 29.80 & 7.17 &  22.21 & .8733 \\
%   w/ relevant keywords $k$ & 40.82 &  13.68 & 29.82 & .8909 \\
%   w/ relevant sentences $s$ & 40.68 & 15.48  & 30.63 & .8901 \\
%   w/ $i$ + $k$ + $s$ & \textbf{48.45} &\textbf{19.53} & \textbf{35.54} & \textbf{.9026} \\

% \bottomrule
% \end{tabular}
% }
% \caption{ \label{tab:res_conditional_citation_generation} 
% The citation generation performance improves with ground-truth citation attributes as conditional input, tested on our SciCCG test set. $\dagger$ represents our own implementation of \citet{xing_automatic_2020}.
% }  
% \end{table}


% For example, given the case shown in Figure \ref{fig:overall-pipeline}, we can extract candidate keywords such as ``unsupervised 3D reconstruction'', ``3D models'', ``2D images'', ``perspective transformer nets'', ``computer vision'', etc.
% In order to extract the most relevant keywords to the target citation sentence, we first encode the contextual text and keywords into embeddings with a text encoder. 
% Using the contextual text as the query, we rank the keywords based the cosine similarity between the keyword embedding and the query embedding. Inspired by \citet{zhong_extractive_2020}, we fine-tune the text encoder so that keywords more relevant to the target citation sentence are ranked to top positions.
% For example, in the case shown in Figure \ref{fig:overall-pipeline}, the desirable ranking of ``perspective transformer nets'' should be higher than that of ``2D images'', since the former is mentioned in the target citation sentence.


% In this section, we first present separately the results of the CCG module and the attribute suggestion module. Then, we evaluate the performance of the entire controlled citation generation pipeline in both automatic mode and user-controlled mode.


We explored two cases. In the first case, we use contextual text as the only input source to generate citation sentences, where we compare PTGEN-Cross \cite{xing_automatic_2020} and 2) BART-large. 
In the second case, we fine-tuned different variants of the BART-large based CCG model, each including different citation attributes as conditions. 

We evaluated the CCG module in an ideal scenario where we assume that the attributes of the citation sentences intended to be generated are known.

when we let BART-large-GCC take the contextual text and the keywords extracted by our keyword extractor as input to generate citation sentences, this ``BART-large-GCC + keyword extractor (ours)'' method achieved higher ROUGE scores than the method BART-large, even though both methods use contextual text as


\begin{itemize}
    \item We proposed a controlled citation generation pipeline with an attribute suggestion module and a conditional text generation module.
    \item We evaluated the controllability of our system in response to different attributes using automated metrics and human evaluation.
    \item We created a large dataset of parsed contextual and attribute-related information for each target citation, which can be used in future studies on controlled citation~generation.
\end{itemize}



%The human evaluation results (Table \ref{tab:res_human_eval}) show that our BART-large-CCG conditional on citation attributes is preferred over the unconditional BART-large model. Sentences generated by BART-large-CCG have higher coherence than BART-large, indicating the good controllability of BART-large-CCG given user-specified attributes, especially keywords. In addition, we observed that in XX\% of the instances, participants selected one or more suggested keywords or sentences, indicating the effectiveness of our attribute suggestion module in recommending possible attributes.

